ClusterLLM: Large Language Models as a Guide for Text Clustering

We introduce ClusterLLM, a novel text clustering framework that leverages feedback from an instruction-tuned large language model, such as ChatGPT. Compared with traditional unsupervised methods that builds upon "small" embedders, ClusterLLM exhibits two intriguing advantages: (1) it enjoys the emergent capability of LLM even if its embeddings are inaccessible; and (2) it understands the user's preference on clustering through textual instruction and/or a few annotated data. First, we prompt ChatGPT for insights on clustering perspective by constructing hard triplet questions <does A better correspond to B than C>, where A, B and C are similar data points that belong to different clusters according to small embedder. We empirically show that this strategy is both effective for fine-tuning small embedder and cost-efficient to query ChatGPT. Second, we prompt ChatGPT for helps on clustering granularity by carefully designed pairwise questions <do A and B belong to the same category>, and tune the granularity from cluster hierarchies that is the most consistent with the ChatGPT answers. Extensive experiments on 14 datasets show that ClusterLLM consistently improves clustering quality, at an average cost of ~$0.6 per dataset. The code will be available at https://github.com/zhang-yu-wei/ClusterLLM.

==> floats/tab_perspective_ablation_app.tex <==

\begin{table*}[ht!]
\centering
\scalebox{0.77}{
\begin{tabular}{l|cccccc|cc}
    \specialrule{0.1em}{0.2em}{0.2em}
    \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Intent Discovery} & \multicolumn{1}{c}{Topic Mining} & \multicolumn{3}{c}{Domain Discovery} & \multicolumn{1}{c}{\multirow{2}{*}{Avg}} & \multicolumn{1}{c}{\multirow{2}{*}{All}}\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-7}
    \multicolumn{1}{c}{} & MTOP(I) & Massive(I) & Reddit & MTOP(D) & Massive(D) & \multicolumn{1}{c}{CLINC(D)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
    \hline
    {\scriptsize Instructor} & 33.35{\tiny (1.32)} & 54.08{\tiny (1.53)} & 54.98{\tiny (1.51)} & 90.56{\tiny (3.34)} & 61.81{\tiny (2.56)} & 52.50{\tiny (2.44)} & 57.88 & 49.90 \\
    {\scriptsize +self-supervise} & 34.06{\tiny (0.64)} & 55.07{\tiny (1.25)} & 55.41{\tiny (0.93)} & 92.12{\tiny (2.66)} & {\bf 62.28}{\tiny (1.55)} & 58.58{\tiny (2.56)} & 59.58 & 51.39 \\
    {\scriptsize +{\model}-random} & 28.05{\tiny (1.69)} & 51.66{\tiny (2.41)} & 54.60{\tiny (2.23)} & 87.0{\tiny (2.27)} & 56.40{\tiny (2.35)} & {\bf 60.27}{\tiny (4.20)} & 56.34 & 48.27 \\
    {\scriptsize +{\model}-GPT3.5} & 35.84{\tiny (2.07)} & {\bf 59.89}{\tiny (2.05)} & 56.79{\tiny (1.90)} & {\bf 93.53}{\tiny (0.10)} & 61.06{\tiny (1.91)} & 52.39{\tiny (1.84)} & 59.91 & 53.09 \\
    {\scriptsize +{\model-GPT4}} & 34.48{\tiny (0.38)} & 59.10{\tiny (1.12)} & 55.38 {\tiny (0.37)} & 92.04{\tiny (2.67)} & 60.16{\tiny (2.97)} & 57.45 {\tiny (2.48)} & 59.77 & 53.22 \\
    {\scriptsize +{\model-GT\&GPT3.5}} & {\bf 36.86}{\tiny (0.42)} & 59.27{\tiny (1.43)} & {\bf 58.33}{\tiny (1.26)} & 92.26{\tiny (3.62)} & 61.65{\tiny (3.50)} & 52.87{\tiny (2.63)} & \bf 60.21 & \bf 53.96\\
    \specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{
More results of ablation study on small-scale datasets. Also see Table~\ref{tab:perspective_ablation}.
}
\label{tab:perspective_ablation_app}
\vspace{-0.3cm}
\end{table*}

==> floats/tab_perspective_ablation_large_2.tex <==

\begin{table*}[ht!]
\centering
\scalebox{0.83}{
\begin{tabular}{l|cccccc|cc}
    \specialrule{0.1em}{0.2em}{0.2em}
    \multicolumn{1}{l}{\multirow{3}{*}{Method}} & \multicolumn{8}{c}{Intent Discovery} & \multicolumn{2}{c}{Emotion} \\
    \cmidrule(lr){2-9} \cmidrule(lr){10-11}
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{Bank77} & \multicolumn{2}{c}{CLINC(I)} & \multicolumn{2}{c}{MTOP(I)} & \multicolumn{2}{c}{Massive(I)} & \multicolumn{2}{c}{GoEmo} \\
    & ACC & NMI & ACC & NMI & ACC & NMI & ACC & NMI & ACC & NMI \\
    \hline
    {\scriptsize Instructor} & 35.53{\tiny (1.05)} & 54.72{\tiny (2.00)} & 55.04 {\tiny (2.69)} & 85.01{\tiny (2.18)} & 56.11{\tiny (5.07)} & 51.74{\tiny (2.97)} & 56.36 & 48.98 \\
    {\scriptsize +self-supervise} & 35.27{\tiny (1.53)} & 58.30{\tiny (1.42)} & 56.45{\tiny (1.59)} & {\bf 89.54}{\tiny (4.56)} & 58.14{\tiny (3.88)} & 50.93{\tiny (4.11)} & 58.11 & 50.30 \\
    {\scriptsize +{\model}-GPT3.5} & 36.80{\tiny (0.83)} & 57.70{\tiny (2.92)} & 55.47{\tiny (2.44)} & 84.08{\tiny (3.34)} & 58.14{\tiny (3.97)} & 50.12{\tiny (4.13)} & 57.05 & \bf 51.21 \\
    {\scriptsize +{\model}-GT\&GPT3.5} & {\bf 37.75}{\tiny (1.64)} & {\bf 58.92}{\tiny (1.80)} & {\bf 57.96}{\tiny (1.96)} & 84.99{\tiny (4.24)} & {\bf 58.55}{\tiny (1.40)} & {\bf 57.08}{\tiny (1.75)} & \bf 59.21 & \bf 52.56\\
    \specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{
Ablation study on clustering quality for large-scale datasets. See more datasets in Table~\ref{tab:perspective_ablation_large_1}.
}
\label{tab:perspective_ablation_large_2}
\end{table*}

==> floats/tab_perspective_analysis_more.tex <==
\definecolor{mygreen}{RGB}{82, 190, 128}
\definecolor{myred}{RGB}{231, 76, 60}
\begin{table*}[ht!]
    \centering
    \scalebox{0.78}{
    \begin{tabular}{c|c|cccccc}
        \specialrule{0.1em}{0.2em}{0.2em}
        Type & Model & MTOP(I) & Massive(I) & Reddit & MTOP(D) & Massive(D) & CLINC(D) \\
        \hline
        \multirow{4}{*}{Random}
        & \#GT Triplets & 102 & 61 & 40 & 184 & 148 & 189 \\
        & Instructor & 98.04 & 88.52 & 80 & 96.74 & 80.41 & 76.72 \\
        & GPT3.5 &  85.29 & 85.25 & 70 & 85.87 & 82.43 & 68.25 \\
        & $\Delta$ & ({\color{myred} -12.75}) & ({\color{myred} -3.27}) & ({\color{myred} -10}) & ({\color{myred} -10.87}) & ({\color{mygreen} +2.02}) & ({\color{myred} -18.47}) \\
        \hline
        \multirow{6}{*}{Entropy-based}
        & \#GT Triplets & 140 & 98 & 92 & 144 & 108 & 208 \\
        & Instructor & 65.74 & 63.56 & 61.98 & 70.31 & 63.82 & 75.06 \\
        & GPT3.5 \dag & 67.41 & 68.76 & 63.28 & 69.79 & 72.09 & 75.78 \\
        & $\Delta$ & ({\color{mygreen} +1.67}) & ({\color{mygreen} +5.20}) & ({\color{mygreen} +1.30}) & ({\color{myred} -0.52}) & ({\color{mygreen} +8.27}) & ({\color{mygreen} +0.72}) \\
        & GPT4 & 76.04 & 74.84 & 67.71 & 72.40 & 70.28 & 74.58 \\
        & $\Delta$ & ({\color{mygreen} +10.30}) & ({\color{mygreen} +11.28}) & ({\color{mygreen} +5.73}) & ({\color{mygreen} +2.09}) & ({\color{mygreen} +6.46}) & ({\color{myred} -0.48}) \\
        \specialrule{0.1em}{0.2em}{0.2em}
    \end{tabular}}
    \caption{Analysis on the triplet accuracy. See other results in Table~\ref{tab:perspective_analysis}.}
    \label{tab:perspective_analysis_more}
\end{table*}

==> floats/tab_perspective_nmi.tex <==

\begin{table*}[ht!]
\centering
\scalebox{0.75}{
\begin{tabular}{l|cccccccc|cc}
    \specialrule{0.1em}{0.2em}{0.2em}
    \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Intent Discovery} & \multicolumn{3}{c}{Type Discovery} & \multicolumn{2}{c}{Topic Mining} & \multicolumn{1}{c}{Emotion} & \multicolumn{1}{c}{\multirow{2}{*}{Avg}} & \multicolumn{1}{c}{\multirow{2}{*}{All}}\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-8} \cmidrule(lr){9-9}
    \multicolumn{1}{c}{} & Bank77 & CLINC(I) & FewRel & FewNerd & FewEvent & StackEx & ArxivS2S & \multicolumn{1}{c}{GoEmo} & \multicolumn{1}{c}{(8)} & \multicolumn{1}{c}{(14)} \\
    \hline
    {\scriptsize Instructor} & 81.43{\tiny (0.61)} & 92.60{\tiny (0.19)} & 57.55{\tiny (0.41)} & 46.12{\tiny (0.54)} & 62.88{\tiny (0.67)} & 65.76{\tiny (0.32)} & 48.04{\tiny (0.39)} & 21.54{\tiny (0.46)} & 59.49 & 63.85 \\
    {\scriptsize self-supervise-I} & 83.31{\tiny (0.59)} & 93.28{\tiny (0.26)} & 57.83{\tiny (0.34)} & 47.25{\tiny (0.47)} & 64.70{\tiny (0.29)} & 66.49{\tiny (0.32)} & 49.41{\tiny (0.17)} & 22.05{\tiny (0.53)} & 60.54 & 65.29 \\
    % {\scriptsize +{\model}-random} & 59.88{\tiny (2.56)} & 74.40{\tiny (0.91)} & 40.65{\tiny (0.89)} & 27.15{\tiny (0.53)} & 44.23{\tiny (1.72)} & 40.81{\tiny (0.94)} & 22.03{\tiny (0.28)} & 28.62{\tiny (1.95)} & 42.22 & 48.27 \\
    {\scriptsize {\model}-I} & {\bf 85.07}{\tiny (0.33)} & {\bf 93.88}{\tiny (0.17)} & {\bf 62.43}{\tiny (0.43)} & {\bf 51.03}{\tiny (0.57)} & {\bf 70.73}{\tiny (0.34)} & {\bf 66.78}{\tiny (0.29)} & {\bf 50.06}{\tiny (0.26)} & {\bf 24.78}{\tiny (0.56)} & \bf 63.10 & \bf 66.58 \\
    % {\scriptsize +{\model-GPT4}} & 69.71{\tiny (1.13)} & 81.91{\tiny (1.20)} & {\bf 48.96}{\tiny (1.14)} & {\bf 37.54}{\tiny (0.54)} & 47.98{\tiny (1.45)} & 46.82{\tiny (0.78)} & 26.16{\tiny (0.22)} & 27.41{\tiny (1.13)} & 48.31 & 53.22 \\
    % {\scriptsize +{\model-GT\&GPT3.5}} & {\bf 71.35}{\tiny (1.97)} & {\bf 84.00} {\tiny (1.04)} & 48.91{\tiny (1.20)} & 37.27{\tiny (0.61)} & {\bf 48.12}{\tiny (1.52)} & {\bf 47.55}{\tiny (1.17)} & 26.14{\tiny (0.57)} & {\bf 30.91}{\tiny (1.16)} & \bf 49.28 & \bf 53.96 \\
    \specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{
NMI score of main results.
}
\label{tab:perspective_nmi}
\vspace{-0.3cm}
\end{table*}

==> floats/tab_perspective_nmi_more.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.83}{
\begin{tabular}{l|cccccc|cc}
    \specialrule{0.1em}{0.2em}{0.2em}
    \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Intent Discovery} & \multicolumn{1}{c}{Topic Mining} & \multicolumn{3}{c}{Domain Discovery} & \multicolumn{1}{c}{\multirow{2}{*}{Avg}} & \multicolumn{1}{c}{\multirow{2}{*}{All}}\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-7}
    \multicolumn{1}{c}{} & MTOP(I) & Massive(I) & Reddit & MTOP(D) & Massive(D) & \multicolumn{1}{c}{CLINC(D)} & \multicolumn{1}{c}{(6)} & \multicolumn{1}{c}{(14)} \\
    \hline
    {\scriptsize Instructor} & 70.63{\tiny (0.27)} & 73.42{\tiny (0.62)} & 62.51{\tiny (0.62)} & 87.30{\tiny (1.53)} & 67.31{\tiny (1.79)} & 56.87{\tiny (2.03)} & 69.67 & 63.85 \\
    {\scriptsize self-supervise-I} & 72.50{\tiny (0.47)} & 72.88{\tiny (0.77)} & 63.45{\tiny (0.86)} & 88.49{\tiny (1.25)} & {\bf 71.53}{\tiny (0.77)} & {\bf 60.84}{\tiny (1.04)} & \bf 71.62 & 65.29 \\
    {\scriptsize {\model}-I} & {\bf 73.52}{\tiny (0.38)} & {\bf 76.96}{\tiny (0.54)} & {\bf 63.87}{\tiny (0.56)} & {\bf 89.36}{\tiny (0.11)} & 68.62{\tiny (0.90)} & 54.98{\tiny (2.08)} & 71.22 & \bf 66.58 \\
    % {\scriptsize +{\model}-GT\&GPT3.5} & {\bf 37.75}{\tiny (1.64)} & {\bf 58.92}{\tiny (1.80)} & {\bf 57.96}{\tiny (1.96)} & 84.99{\tiny (4.24)} & {\bf 58.55}{\tiny (1.40)} & {\bf 57.08}{\tiny (1.75)} & \bf 59.21 & \bf 52.56\\
    \specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{
NMI score of main results.
}
\label{tab:perspective_nmi_more}
\vspace{-0.3cm}
\end{table*}

==> floats/tab_perspective_sota_app.tex <==

\begin{table*}[ht!]
\centering
\scalebox{0.78}{
\begin{tabular}{c|ccccc|c}
    \specialrule{0.1em}{0.2em}{0.2em}
    \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Intent Discovery} & \multicolumn{1}{c}{Topic Mining} & \multicolumn{3}{c}{Domain Discovery} & \multicolumn{1}{c}{\multirow{2}{*}{Avg}} & \multicolumn{1}{c}{\multirow{2}{*}{All}}\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-5} \cmidrule(lr){6-8}
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & MTOP(I) & Massive(I) & Reddit & MTOP(D) & Massive(D) & \multicolumn{1}{c}{CLINC(D)} & \multicolumn{1}{c}{(6)} & \multicolumn{1}{c}{(14)}\\
    \hline
    % \multirow{4}{*}{\ding{51}}
    % & {\small ORCA}{\tiny ~\cite{cao2022openworld}}{\small \dag} \\
    % &{\small Contrast}{\tiny ~\cite{vaze2022gcd}}{\small \dag} & 29.25{\tiny (0.90)} & 33.07{\tiny (2.26)} & 19.57{\tiny (0.82)} & - & - & - & - & - \\
    % &{\small DAC}{\tiny ~\cite{Zhang_Xu_Lin_Lyu_2021}} & 31.43{\tiny (1.42)} & 34.45{\tiny (3.57)} & 16.80{\tiny (2.72)} & - & - & - & - & - \\
    % &{\small DPN}{\tiny ~\cite{an2022dpn}} & 33.64{\tiny (2.93)} & 33.86{\tiny (4.50)} & 14.69{\tiny (1.36)} & - & - & - & - & -\\
    % &{\small CLNN}{\tiny ~\cite{zhang-etal-2022-new}} & 29.77{\tiny (1.07)} & 46.22{\tiny (1.63)} & 29.01{\tiny (4.00)} & - & - & - & - & - \\
    % \hline
    % \multirow{10}{*}{\ding{55}}
    {\small \underline{E}5}{\tiny ~\cite{wang2022text}} & 33.54{\tiny (0.92)} & 52.52{\tiny (0.62)} & 39.03{\tiny (0.62)} & 91.23{\tiny (1.23)} & {\bf 63.70}{\tiny (0.86)} & 59.64{\tiny (2.73)} & 56.61 & 47.70 \\
    {\small SCCL-\underline{E}}{\tiny ~\cite{zhang-etal-2021-supporting}} & 33.82{\tiny (1.07)} & 54.48{\tiny (1.80)} & 44.45{\tiny (0.79)} & 92.28{\tiny (0.18)} & 61.22{\tiny (1.15)} & 59.88{\tiny (2.74)} & 57.69 & 48.87\\
    {\small self-supervise-\underline{E}} & 33.81{\tiny (0.70)} & 54.23{\tiny (1.57)} & 48.69{\tiny (2.40)} & 91.40{\tiny (4.61)} & 61.79{\tiny (2.50)} & 57.29{\tiny (2.51)} & 57.87 & 49.87 \\
    {\small {\model}-\underline{E}} & 34.66{\tiny (0.74)} & 57.09{\tiny (1.91)} & 47.72{\tiny (1.58)} & 89.18{\tiny (5.25)} & 60.73{\tiny (2.81)} & 56.25{\tiny (2.94)} & 57.61 & 50.93 \\
    {\small {\model}-\underline{E}-iter} & {\bf 37.22}{\tiny (1.18)} & 56.08{\tiny (1.01)} & 49.05{\tiny (1.15)} & 89.58{\tiny (5.08)} & 58.63{\tiny (1.32)} & {\bf 60.84}{\tiny (2.88)} & 58.57 & 52.40\\\cline{2-10}
    {\small \underline{I}nstructor}{\tiny ~\cite{INSTRUCTOR}} & 33.35{\tiny (1.32)} & 54.08{\tiny (1.53)} & 54.98{\tiny (1.51)} & 90.56{\tiny (3.34)} & 61.81{\tiny (2.56)} & 52.50{\tiny (2.44)} & 57.88 & 49.90 \\
    {\small SCCL-\underline{I}}{\tiny ~\cite{zhang-etal-2021-supporting}} & 34.28{\tiny (0.58)} & 54.05{\tiny (1.05)} & 53.66{\tiny (0.94)} & 89.08{\tiny (3.77)} & 61.34{\tiny (2.77)} & 54.22{\tiny (3.15)} & 57.77 & 50.73 \\
    {\small self-supervise-\underline{I}} & 34.06{\tiny (0.64)} & 55.07{\tiny (1.25)} & 55.41{\tiny (0.93)} & 92.12{\tiny (2.66)} & 62.28{\tiny (1.55)} & 58.58{\tiny (2.56)} & 59.58 & 51.39 \\
    {\small {\model}-\underline{I}} & 35.84{\tiny (2.07)} & 59.89{\tiny (2.05)} & 56.79{\tiny (1.90)} & {\bf 93.53}{\tiny (0.10)} & 61.06{\tiny (1.91)} & 52.39{\tiny (1.84)} & \bf 59.91 & 53.09 \\
    {\small {\model-\underline{I}-iter}} & 35.04{\tiny (0.97)} & {\bf 60.69}{\tiny (0.96)} & {\bf 57.02}{\tiny (0.87)} & 92.13{\tiny (3.81)} & 60.85{\tiny (4.33)}  & 51.82{\tiny (1.91)} & 59.59 & \bf 53.99 \\
    \specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{
The setting is the same as in Table~\ref{tab:perspective_sota}.
}
\label{tab:perspective_sota_app}
\end{table*}
